Exploring Landscapes for Better Minima along Valleys

Finding lower and better-generalizing minima is crucial for deep learning. However, most existing optimizers stop searching the parameter space once they reach a local minimum. Given the complex geometric properties of the loss landscape, it is difficult to guarantee that such a point is the lowest or provides the best generalization. To address this, we propose an adaptor "E" for gradient-based optimizers. The adapted optimizer tends to continue exploring along landscape valleys (areas with low and nearly identical losses) in order to search for potentially better local minima even after reaching a local minimum. This approach increases the likelihood of finding a lower and flatter local minimum, which is often associated with better generalization. We also provide a proof of convergence for the adapted optimizers in both convex and non-convex scenarios for completeness. Finally, we demonstrate their effectiveness in an important but notoriously difficult training scenario, large-batch training, where Lamb is the benchmark optimizer. Our testing results show that the adapted Lamb, ALTO, increases the test accuracy (generalization) of the current state-of-the-art optimizer by an average of 2.5% across a variety of large-batch training tasks. This work potentially opens a new research direction in the design of optimization algorithms.

==> paperstyle.tex <==
\ProvidesPackage{tongstyle}[2024/12/03 Tong style]
\usepackage{ifthen}  % using if
\usepackage{pgffor}  % using for

\usepackage{enumitem} % enumerate enviornment and item
\usepackage{bm} % bolding any math character, e.g. \bm{\alpha}
\usepackage{xspace} % \newcommand{\R}{\mathbb{R}\xspace}  % Automatically adds space after \R

\usepackage[utf8]{inputenc} % allow utf-8 input
\usepackage[T1]{fontenc}    % use 8-bit T1 fonts
\usepackage{wrapfig}
\usepackage{amsmath} % math enviornment
\usepackage{amssymb} % math symbol
\usepackage{mathtools} % math tools
\usepackage{amsthm} % math theorem, lemma, definition
\usepackage{amsfonts}       % blackboard math symbols
\definecolor{citecolor}{HTML}{696FAD}
\definecolor{tablered}{HTML}{F5E6E9}
\definecolor{tablegreen}{HTML}{E2E6E1}
\definecolor{tableyellow}{HTML}{F9F2EB}
\definecolor{tableblue}{HTML}{CDD4DF}

\definecolor{MyBlue}{rgb}{0.46, 0.50, 0.61}
\definecolor{MyDarkBlue}{rgb}{0,0.08,0.8}
\definecolor{MyDarkGreen}{RGB}{45,155,45}
\definecolor{MyDarkRed}{rgb}{0.8,0.02,0.02}
\definecolor{MyOrange}{rgb}{1.0, 0.4, 0.2}
\definecolor{MyPurple}{RGB}{111,0,255}
\definecolor{MyRed}{rgb}{0.8,0.0,0.0}
\definecolor{MyGold}{rgb}{0.75,0.6,0.12}
\definecolor{MyDarkgray}{rgb}{0.66, 0.66, 0.66}
\definecolor{MyBrown}{rgb}{0.65, 0.16, 0.16}
\definecolor{MyMutedRose}{rgb}{0.58, 0.29, 0.35}
\definecolor{JiayuanColor}{rgb}{0.60,0.43,0.48}
\definecolor{erranColor}{rgb}{24, 40, 113}
\usepackage[pagebackref=true,breaklinks=true,colorlinks,citecolor=citecolor,anchorcolor=citecolor,linkcolor=citecolor,urlcolor=citecolor,bookmarks=false]{hyperref}     % hyperlinks
\usepackage{url}            % adding URL, e.g.\url{https://}
\usepackage{nicefrac}       % compact symbols for inline 1/2, e.g. \nicefrac{1}{2}.
\usepackage{xcolor}         % setting colors for text and tables
\usepackage{colortbl}
\usepackage[framemethod=tikz]{mdframed}

\usepackage[capitalize,noabbrev,nameinlink]{cleveref}
\crefname{assumption}{Assumption}{Assumptions}
% \crefname{equation}{Eq.}{Eqs.}
\crefname{observation}{Observation}{Observations}

\usepackage{pifont} % ding{} Special Characters
\usepackage{multirow} % multi-row
\usepackage{multicol} % multi-column
\usepackage[toc,page,header]{appendix} % appendix
\usepackage{tocloft}  % table of contents, graph and table list
\usepackage{minitoc}

\renewcommand{\contentsname}{}
\renewcommand{\cftsecleader}{\cftdotfill{\cftdotsep}}
\usepackage{algorithm}
% \usepackage{algorithmic}
\usepackage{algpseudocode} % 算法伪代码宏包
\newcommand{\numberthis}[1]{%
    \refstepcounter{equation}% 增加方程计数器
    \label{#1}% 添加标签
    \tag{\theequation}% 手动编号当前行
}
\usepackage[capitalize,noabbrev,nameinlink]{cleveref}
\usepackage{microtype}      % better typesetting
\usepackage{graphicx}       % adjust figure
% \usepackage[numbers]{natbib}
% \usepackage{subfigure}
\usepackage{subcaption}    % for subfigure and subcaption
\usepackage{booktabs}       % professional-quality tables
\usepackage{fontawesome5}   % logo benenth title
\usepackage[most]{tcolorbox}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% THEOREMS
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\theoremstyle{plain}
\newtheorem{theorem}{Theorem}
\newtheorem{proposition}{Proposition}[section]
\newtheorem{lemma}{Lemma}
\newtheorem{corollary}{Corollary}[section]
\theoremstyle{definition}
\newtheorem{definition}{Definition}[section]
\newtheorem{challenge}{Challenge}[section]
\newtheorem{observation}{Observation}[section]
\newtheorem{assumption}{Assumption}[section]
\theoremstyle{remark}
\newtheorem{remark}{Remark}[section]

\newcommand{\acronym}{ALTO}
%----- bold fonts -----%

\newcommand{\ba}{\mathbf{a}}
\newcommand{\bb}{\mathbf{b}}
\newcommand{\bc}{\mathbf{c}}
\newcommand{\bd}{\mathbf{d}}
\newcommand{\be}{\mathbf{e}}
% \newcommand{\bf}{\mathbf{f}}
\newcommand{\bg}{\mathbf{g}}
\newcommand{\bh}{\mathbf{h}}
\newcommand{\bi}{\mathbf{i}}
\newcommand{\bj}{\mathbf{j}}
\newcommand{\bk}{\mathbf{k}}
\newcommand{\bl}{\mathbf{l}}
% \newcommand{\bm}{\mathbf{m}}
\newcommand{\bn}{\mathbf{n}}
\newcommand{\bo}{\mathbf{o}}
\newcommand{\bp}{\mathbf{p}}
\newcommand{\bq}{\mathbf{q}}
\newcommand{\br}{\mathbf{r}}
\newcommand{\bs}{\mathbf{s}}
\newcommand{\bt}{\mathbf{t}}
\newcommand{\bu}{\mathbf{u}}
\newcommand{\bv}{\mathbf{v}}
\newcommand{\bw}{\mathbf{w}}
\newcommand{\bx}{\mathbf{x}}
\newcommand{\by}{\mathbf{y}}
\newcommand{\bz}{\mathbf{z}}

% % \newcommand{\ab}{\mathbf{a}}
% \newcommand{\bbb}{\mathbf{b}}
% \newcommand{\cbb}{\mathbf{c}}
% \newcommand{\db}{\mathbf{d}}
% \newcommand{\eb}{\mathbf{e}}
% \newcommand{\fb}{\mathbf{f}}
% \newcommand{\gb}{\mathbf{g}}
% \newcommand{\hb}{\mathbf{h}}
% \newcommand{\ib}{\mathbf{i}}
% \newcommand{\jb}{\mathbf{j}}
% \newcommand{\kb}{\mathbf{k}}
% \newcommand{\lb}{\mathbf{l}}
% \newcommand{\mb}{\mathbf{m}}
% \newcommand{\nbb}{\mathbf{n}}
% \newcommand{\ob}{\mathbf{o}}
% \newcommand{\pb}{\mathbf{p}}
% \newcommand{\qb}{\mathbf{q}}
% % \newcommand{\rb}{\mathbf{r}}
% \newcommand{\sbb}{\mathbf{s}}
% \newcommand{\tb}{\mathbf{t}}
% \newcommand{\ub}{\mathbf{u}}
% % \newcommand{\vb}{\mathbf{v}}
% \newcommand{\wb}{\mathbf{w}}
% \newcommand{\xb}{\mathbf{x}}
% \newcommand{\yb}{\mathbf{y}}
% \newcommand{\zb}{\mathbf{z}}

\newcommand{\ab}{\bm{a}}
\newcommand{\bbb}{\bm{b}}
\newcommand{\cb}{\bm{c}}
\newcommand{\db}{\bm{d}}
\newcommand{\eb}{\bm{e}}
\newcommand{\fb}{\bm{f}}
\newcommand{\gb}{\bm{g}}
\newcommand{\hb}{\bm{h}}
\newcommand{\ib}{\bmf{i}}
\newcommand{\jb}{\bm{j}}
\newcommand{\kb}{\bm{k}}
\newcommand{\lb}{\bm{l}}
\newcommand{\mb}{\bm{m}}
\newcommand{\nb}{\bm{n}}
\newcommand{\ob}{\bm{o}}
\newcommand{\pb}{\bm{p}}
\newcommand{\qb}{\bm{q}}
\newcommand{\rb}{\bm{r}}
% \newcommand{\sb}{\bm{s}}
\newcommand{\tb}{\bm{t}}
\newcommand{\ub}{\bm{u}}
\newcommand{\vb}{\bm{v}}
\newcommand{\wb}{\bm{w}}
\newcommand{\xb}{\bm{x}}
\newcommand{\yb}{\bm{y}}
\newcommand{\zb}{\bm{z}}

% \newcommand{\ba}{\bm{a}}
% \newcommand{\bb}{\bm{b}}
% \newcommand{\bc}{\bm{c}}
% \newcommand{\bd}{\bm{d}}
% \newcommand{\be}{\bm{e}}
% \newcommand{\bbf}{\bm{f}}
% \newcommand{\bg}{\bm{g}}
% \newcommand{\bh}{\bm{h}}
% \newcommand{\bi}{\bmf{i}}
% \newcommand{\bj}{\bm{j}}
% \newcommand{\bk}{\bm{k}}
% \newcommand{\bl}{\bm{l}}
% \newcommand{\bbm}{\bm{m}}
% \newcommand{\bn}{\bm{n}}
% \newcommand{\bo}{\bm{o}}
% \newcommand{\bp}{\bm{p}}
% \newcommand{\bq}{\bm{q}}
% \newcommand{\br}{\bm{r}}
% \newcommand{\bs}{\bm{s}}
% \newcommand{\bt}{\bm{t}}
% \newcommand{\bu}{\bm{u}}
% \newcommand{\bv}{\bm{v}}
% \newcommand{\bw}{\bm{w}}
% \newcommand{\bx}{\bm{x}}
% \newcommand{\by}{\bm{y}}
% \newcommand{\bz}{\bm{z}}


\newcommand{\bA}{\mathbf{A}}
\newcommand{\bB}{\mathbf{B}}
\newcommand{\bC}{\mathbf{C}}
\newcommand{\bD}{\mathbf{D}}
\newcommand{\bE}{\mathbf{E}}
\newcommand{\bF}{\mathbf{F}}
\newcommand{\bG}{\mathbf{G}}
\newcommand{\bH}{\mathbf{H}}
\newcommand{\bI}{\mathbf{I}}
\newcommand{\bJ}{\mathbf{J}}
\newcommand{\bK}{\mathbf{K}}
\newcommand{\bL}{\mathbf{L}}
\newcommand{\bM}{\mathbf{M}}
\newcommand{\bN}{\mathbf{N}}
\newcommand{\bO}{\mathbf{O}}
\newcommand{\bP}{\mathbf{P}}
\newcommand{\bQ}{\mathbf{Q}}
\newcommand{\bR}{\mathbf{R}}
\newcommand{\bS}{\mathbf{S}}
\newcommand{\bT}{\mathbf{T}}
\newcommand{\bU}{\mathbf{U}}
\newcommand{\bV}{\mathbf{V}}
\newcommand{\bW}{\mathbf{W}}
\newcommand{\bX}{\mathbf{X}}
\newcommand{\bY}{\mathbf{Y}}
\newcommand{\bZ}{\mathbf{Z}}

% \newcommand{\Ab}{\mathbf{A}}
% \newcommand{\Bb}{\mathbf{B}}
% \newcommand{\Cb}{\mathbf{C}}
% \newcommand{\Db}{\mathbf{D}}
% \newcommand{\Eb}{\mathbf{E}}
% \newcommand{\Fb}{\mathbf{F}}
% \newcommand{\Gb}{\mathbf{G}}
% \newcommand{\Hb}{\mathbf{H}}
% \newcommand{\Ib}{\mathbf{I}}
% \newcommand{\Jb}{\mathbf{J}}
% \newcommand{\Kb}{\mathbf{K}}
% \newcommand{\Lb}{\mathbf{L}}
% \newcommand{\Mb}{\mathbf{M}}
% \newcommand{\Nb}{\mathbf{N}}
% \newcommand{\Ob}{\mathbf{O}}
% \newcommand{\Pb}{\mathbf{P}}
% \newcommand{\Qb}{\mathbf{Q}}
% \newcommand{\Rb}{\mathbf{R}}
% \newcommand{\Sbb}{\mathbf{S}}
% \newcommand{\Tb}{\mathbf{T}}
% \newcommand{\Ub}{\mathbf{U}}
% \newcommand{\Vb}{\mathbf{V}}
% \newcommand{\Wb}{\mathbf{W}}
% \newcommand{\Xb}{\mathbf{X}}
% \newcommand{\Yb}{\mathbf{Y}}
% \newcommand{\Zb}{\mathbf{Z}}

\newcommand{\Ab}{\bm{A}}
\newcommand{\Bb}{\bm{B}}
\newcommand{\Cb}{\bm{C}}
\newcommand{\Db}{\bm{D}}
\newcommand{\Eb}{\bm{E}}
\newcommand{\Fb}{\bm{F}}
\newcommand{\Gb}{\bm{G}}
\newcommand{\Hb}{\bm{H}}
\newcommand{\Ib}{\bm{I}}
\newcommand{\Jb}{\bm{J}}
\newcommand{\Kb}{\bm{K}}
\newcommand{\Lb}{\bm{L}}
\newcommand{\Mb}{\bm{M}}
\newcommand{\Nb}{\bm{N}}
\newcommand{\Ob}{\bm{O}}
\newcommand{\Pb}{\bm{P}}
\newcommand{\Qb}{\bm{Q}}
\newcommand{\Rb}{\bm{R}}
\newcommand{\Sb}{\bm{S}}
\newcommand{\Tb}{\bm{T}}
\newcommand{\Ub}{\bm{U}}
\newcommand{\Vb}{\bm{V}}
\newcommand{\Wb}{\bm{W}}
\newcommand{\Xb}{\bm{X}}
\newcommand{\Yb}{\bm{Y}}
\newcommand{\Zb}{\bm{Z}}

% \newcommand{\bA}{\bm{A}}
% \newcommand{\bB}{\bm{B}}
% \newcommand{\bC}{\bm{C}}
% \newcommand{\bD}{\bm{D}}
% \newcommand{\bE}{\bm{E}}
% \newcommand{\bF}{\bm{F}}
% \newcommand{\bG}{\bm{G}}
% \newcommand{\bH}{\bm{H}}
% \newcommand{\bI}{\bm{I}}
% \newcommand{\bJ}{\bm{J}}
% \newcommand{\bK}{\bm{K}}
% \newcommand{\bL}{\bm{L}}
% \newcommand{\bM}{\bm{M}}
% \newcommand{\bN}{\bm{N}}
% \newcommand{\bO}{\bm{O}}
% \newcommand{\bP}{\bm{P}}
% \newcommand{\bQ}{\bm{Q}}
% \newcommand{\bR}{\bm{R}}
% \newcommand{\bS}{\bm{S}}
% \newcommand{\bT}{\bm{T}}
% \newcommand{\bU}{\bm{U}}
% \newcommand{\bV}{\bm{V}}
% \newcommand{\bW}{\bm{W}}
% \newcommand{\bX}{\bm{X}}
% \newcommand{\bY}{\bm{Y}}
% \newcommand{\bZ}{\bm{Z}}

%----- calligraphic fonts -----%

\newcommand{\cA}{\mathcal{A}}
\newcommand{\cB}{\mathcal{B}}
\newcommand{\cC}{\mathcal{C}}
\newcommand{\cD}{\mathcal{D}}
\newcommand{\cE}{\mathcal{E}}
\newcommand{\cF}{\mathcal{F}}
\newcommand{\cG}{\mathcal{G}}
\newcommand{\cH}{\mathcal{H}}
\newcommand{\cI}{\mathcal{I}}
\newcommand{\cJ}{\mathcal{J}}
\newcommand{\cK}{\mathcal{K}}
\newcommand{\cL}{\mathcal{L}}
\newcommand{\cM}{\mathcal{M}}
\newcommand{\cN}{\mathcal{N}}
\newcommand{\cO}{\mathcal{O}}
\newcommand{\cP}{\mathcal{P}}
\newcommand{\cQ}{\mathcal{Q}}
\newcommand{\cR}{\mathcal{R}}
\newcommand{\cS}{\mathcal{S}}
\newcommand{\cT}{\mathcal{T}}
\newcommand{\cU}{\mathcal{U}}
\newcommand{\cV}{\mathcal{V}}
\newcommand{\cW}{\mathcal{W}}
\newcommand{\cX}{\mathcal{X}}
\newcommand{\cY}{\mathcal{Y}}
\newcommand{\cZ}{\mathcal{Z}}


%----- blackboard bold fonts-----%

\newcommand{\BB}{\mathbb{B}}
\newcommand{\CC}{\mathbb{C}}
\newcommand{\EE}{\mathbb{E}}
\newcommand{\VV}{\mathbb{V}}
\newcommand{\HH}{\mathbb{H}}
\newcommand{\II}{\mathbb{I}}
\newcommand{\KK}{\mathbb{K}}
\newcommand{\LL}{\mathbb{L}}
\newcommand{\MM}{\mathbb{M}}
\newcommand{\NN}{\mathbb{N}}
\newcommand{\PP}{\mathbb{P}}
\newcommand{\QQ}{\mathbb{Q}}
\newcommand{\RR}{\mathbb{R}}
\newcommand{\SSS}{\mathbb{S}}
\newcommand{\XX}{\mathbb{X}}
\newcommand{\YY}{\mathbb{Y}}
\newcommand{\ZZ}{\mathbb{Z}}
\newcommand{\OOmega}{\mathbb{\Omega}}


%----- bold greek fonts -----%

\newcommand{\bmeta}{\bm{\eta}}

\newcommand{\balpha}{\bm{\alpha}}
\newcommand{\bbeta}{\bm{\beta}}
\newcommand{\bgamma}{\bm{\gamma}}
\newcommand{\bepsilon}{\bm{\epsilon}}
\newcommand{\bvarepsilon}{\bm{\varepsilon}}
\newcommand{\bzeta}{\bm{\zeta}}
\newcommand{\btheta}{\bm{\theta}}
\newcommand{\bvartheta}{\bm{\vartheta}}
\newcommand{\bkappa}{\bm{\kappa}}
\newcommand{\blambda}{\bm{\lambda}}
\newcommand{\bmu}{\bm{\mu}}
\newcommand{\bnu}{\bm{\nu}}
\newcommand{\bxi}{\bm{\xi}}
\newcommand{\bpi}{\bm{\pi}}
\newcommand{\bvarpi}{\bm{\varpi}}
\newcommand{\brho}{\bm{\varrho}}
\newcommand{\bsigma}{\bm{\sigma}}
\newcommand{\bvarsigma}{\bm{\varsigma}}
\newcommand{\btau}{\bm{\tau}}
\newcommand{\bupsilon}{\bm{\upsilon}}
\newcommand{\bphi}{\bm{\phi}}
\newcommand{\bvarphi}{\bm{\varphi}}
\newcommand{\bchi}{\bm{\chi}}
\newcommand{\bpsi}{\bm{\psi}}
\newcommand{\bomega}{\bm{\omega}}

\newcommand{\bGamma}{\bm{\Gamma}}
\newcommand{\bDelta}{\bm{\Delta}}
\newcommand{\bTheta}{\bm{\Theta}}
\newcommand{\bLambda}{\bm{\Lambda}}
\newcommand{\bXi}{\bm{\Xi}}
\newcommand{\bPi}{\bm{\Pi}}
\newcommand{\bSigma}{\bm{\Sigma}}
\newcommand{\bUpsilon}{\bm{\Upsilon}}
\newcommand{\bPhi}{\bm{\Phi}}
\newcommand{\bPsi}{\bm{\Psi}}
\newcommand{\bOmega}{\bm{\Omega}}


%----- Some standard definitions -----%

% \newcommand{\argmin}{\mathop{\mathrm{argmin}}}
% \newcommand{\argmax}{\mathop{\mathrm{argmax}}}
\newcommand{\minimize}{\mathop{\mathrm{minimize}}}

% \newcommand{\sign}{\mathop{\mathrm{sign}}}
\newcommand{\tr}{\mathop{\mathrm{tr}}}

% \DeclareMathOperator{\Var}{{\rm Var}}
\DeclareMathOperator{\Cor}{\rm Corr}
% \DeclareMathOperator{\Cov}{\rm Cov}
\DeclareMathOperator{\ind}{\mathds{1}}  % Indicator
\newcommand{\smallfrac}[2]{{\textstyle \frac{#1}{#2}}}  
                                                        
\newcommand*{\zero}{{\bm 0}}
\newcommand*{\one}{{\bm 1}}

\newcommand{\diag}{{\rm diag}}

% \newcommand{\theHalgorithm}{\arabic{algorithm}}
\renewcommand{\algorithmicrequire}{\textbf{Input:}}
\renewcommand{\algorithmicensure}{\textbf{Output:}}
\DeclareMathOperator*{\argmin}{arg\,min}
\DeclareMathOperator*{\argmax}{arg\,max}
\newcommand*{\T}{^{\mkern-1.5mu\mathsf{T}}} % e.g. $A\T$
\DeclareMathOperator*{\var}{Var}


% Abbr
\def\ie{\textit{i.e.,~}}
\def\eg{\textit{e.g.,~}}
\def\etc{\textit{etc}}
\def\etal{\textit{et al.~}}
\def\wrt{\textit{w.r.t.~}}
\def\vs{\textit{v.s.~}}
\def\resp{\textit{resp.~}}
\def\sota{state-of-the-art~}



% Todonotes is useful during development; simply uncomment the next line
%    and comment out the line below the next line to turn off comments
%\usepackage[disable,textsize=tiny]{todonotes}
\usepackage[textsize=tiny]{todonotes}

% Typeset listings.
\usepackage{newfloat}
\usepackage{listings}
\DeclareCaptionStyle{ruled}{labelfont=normalfont,labelsep=colon,strut=off} % DO NOT CHANGE THIS
\lstset{%
	basicstyle={\footnotesize\ttfamily},% footnotesize acceptable for monospace
	numbers=left,numberstyle=\footnotesize,xleftmargin=2em,% show line numbers, remove this entire line if you don't want the numbers.
	aboveskip=0pt,belowskip=0pt,%
	showstringspaces=false,tabsize=2,breaklines=true}
\floatstyle{ruled}
\newfloat{listing}{tb}{lst}{}
\floatname{listing}{Listing}
%
% Keep the \pdfinfo as shown here. There's no need
% for you to add the /Title and /Author tags.
\pdfinfo{
/TemplateVersion (2025.1)
}

%Set section index depth. e.g. 1.2, 2.3.
\setcounter{secnumdepth}{2} 


\AtBeginDocument{\addtocontents{toc}{\protect\setcounter{tocdepth}{-1}}}
% tong style appendix
\newcommand{\Appendix}{%
  \newpage
  \section*{\begin{center}\LARGE Appendix\end{center}} % Appendix title
  \addcontentsline{toc}{section}{Appendix} % Add to table of contents
  \tableofcontents
  % Now start your appendix sections
  \addtocontents{toc}{\protect\setcounter{tocdepth}{2}}
  % Content of this section
  \appendix
  \newpage
  \setcounter{theorem}{0}
  \newpage 
}

\newtcolorbox{onebox}[2][]{
enhanced, 
center title,
left*=0pt, right*=0pt,
boxsep=2pt, left=5pt, right=5pt,
skin first=enhanced,
skin middle=enhanced,
skin last=enhanced,
colframe = MyBlue!90,
colback  = MyBlue!10,
fonttitle=\bfseries\rmfamily\fontfamily{phv}\selectfont,
title={\footnotesize\strut{#2}  \refstepcounter{subsubsection} \addcontentsline{toc}{subsubsection}{\string\numberline{\thesubsubsection}#2}
},
#1
}



% newcommand can be used like this:
% \newcommand{\R}{\mathbb{R}}  % customize a command "\R" as "\mathbb{R}"
% \newcommand{\veca}[1]{\mathbf{#1}}  % customize a command "\veca{}" accepting a parameter in "{}"
% \newcommand{\myfrac}[2]{\frac{#1}{#2}}  % customize a command "\myfrac{}{}" accepting a parameter in "{}{}"
% \newcommand{\vect}[3]{\mathbf{#1} \times \mathbf{#2} \times \mathbf{#3}}  %  customize a command "\vect{}{}{}" accepting three parameters in "{}{}{}"
% \newcommand{\mytext}[2][default]{Text: #1, More text: #2} % customize a command "\mytext{}{}" accepting two parameters in "{}{}", the default is a default parameter for #1

% \def can be used like this:
% \def\mycommand#1{%
%   \ifx\empty#1\empty
%     Text: Default
%   \else
%     Text: #1
%   \fi
% } where \mycommand is a function name (command), #1 is a parameter, what is in {} is definition of the function \mycommand

% \input and \include can be used like this:
% \input{xxx.tex}: this will import xxx.tex file at the command \input{xxx.tex} as we just put contents of xxx.tex there directly.
% \include{xxx.tex}: this will import xxx.tex file at the command \input{xxx.tex} there, but in a newpage.

% \newenvironment can be used like this:
% \newenvironment{name}{begin}{end}

% "if" can be used like this:
% \ifthenelse{\value{section}=1}{This is section 1.}{This is not section 1.}

% "for" can be used like this:
% \foreach \x in {1, 2, 3} {
%   Number: \x\par
% }

% \newwrite \openout \closeout can be used like this:
% \newwrite\myfile  % define a new varible \myfile
% \openout\myfile=output.txt  % open \myfile=output.txt
% \write\myfile{This is some content for the file.}  % write done things in {} to \myfile
% \closeout\myfile  % close \myfile


% \DeclareMathOperator* can be used like this:
% \DeclareMathOperator*{command_name}{output_for_display}, where * means we can use adaptive superscript and subscript.

% In \section*, \equation* , etc., * means these entries are not numbered.

%\addcontentsline, \addcontents are build-in commands
% toc, lof, lot are build-in file table of contents, list of figures and list of tables.


% \setcounter, \addtocounter, \value can be used like this:
% \setcounter{section}{2}  % setting the varible "section index" 2, and then the "section index" will increase from 2.
% \addtocounter{section}{1}  % adding 2 to the varible "section index" thereafter.
% \value{section}  % getting the value of the varible "section index" there.
